WPaxos: Wide Area Network Flexible Consensus

WPaxos is a multileader Paxos protocol that provides low-latency and high-throughput consensus across wide-area network (WAN) deployments. WPaxos uses multileaders, and partitions the object-space among these multileaders. Unlike statically partitioned multiple Paxos deployments, WPaxos is able to adapt to the changing access locality through object stealing. Multiple concurrent leaders coinciding in different zones steal ownership of objects from each other using phase-1 of Paxos, and then use phase-2 to commit update-requests on these objects locally until they are stolen by other leaders. To achieve fast phase-2 commits, WPaxos adopts the flexible quorums idea in a novel manner, and appoints phase-2 acceptors to be close to their respective leaders. We implemented WPaxos and evaluated it on WAN deployments across 5 AWS regions. The dynamic partitioning of the object-space and emphasis on zone-local commits allow WPaxos to significantly outperform both partitioned Paxos deployments and leaderless Paxos approaches.

==> consistency.tex <==
\subsection{Consistency}

WPaxos consistency guarantees are on par with other similar protocols, such as EPaxos, solving the generalized consensus problem, first introduced in 2005~\cite{generalizedconsensus}. Generalized consensus relaxes the consensus requirement by allowing non-interfering commands to be processed concurrently. Generalized consensus no longer has a totally ordered set of command, instead only conflicting commands need to be ordered with respect to each other, making the command log a partially ordered set. WPaxos maintains separate logs for each object and provides per-object linearizability. Moreover, for multi-object minitransactional commands our protocol solves the generalized consensus and provides strict serializability. We can collate or serialize the logs together, establishing the order of interfering commands by comparing the slot numbers of the objects in the commands, as shown in Figure~\ref{fig:wpaxos_log_collate}. This ordering happens naturally as the commands cannot get executed before the previous slots for all objects in the command are executed. The serializability we achieve through the log collation along with the per-object linearizability of all objects in the system make WPaxos a strictly serializable protocol~\cite{linearizability}.

\begin{figure}[!t]
\centering
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\linewidth]{figures/wpaxos_log_collate_a.pdf}
\caption{Logs for 3 objects $A$, $B$, and $C$. Dashed box encompasses multi-object commands.} \label{fig:wpaxos_log_collate_a}
\end{subfigure}
\hspace*{\fill} % separation between the subfigures
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\linewidth]{figures/wpaxos_log_collate_b.pdf}
\caption{Object logs are serialized. Multi-object transactions are ordered based on the slot numbers} \label{fig:wpaxos_log_collate_b}
\end{subfigure}
\caption{Log Serialization for objects $A$, $B$, and $C$.}
\label{fig:wpaxos_log_collate}
\end{figure}


==> object_stealing.tex <==
% Subsection Object Ste.  ling
%\subsection{Object Stealing}

Object stealing is part of core WPaxos protocol: in the normal case, the object's leadership changes (with a higher ballot number) in just a single phase-1 execution performed on one of the $Q_1$ quorums. In contrast to the simplicity and agility of object stealing in WPaxos, object relocation in other systems require integration of another service, such as movedir in Spanner~\cite{spanner}, or performing multiple reconfiguration or coordination steps as in Vertical Paxos~\cite{verticalpaxos}.

Vertical Paxos depends on a reliable master service that overseeing configuration changes. Object relocation involves configuration change in the node responsible for processing commands on that object. When a node in a different region attempts to become the own of the object, When a node in a different region attempts to become the owner of the object, it must first contact the reconfiguration master to obtain the current ballot number and next ballot to be used. The new leader then must complete phase-1 of Paxos on the old configuration to learn the previous commands. Upon finishing the phase-1, the new leader can commit any uncommitted slots with its own set of acceptors. At the same time the new leader notifies the master of completing phase-1 with its ballot. Only after the master replies and activates the new configuration, the leader can start serving user requests. This process can be extended to multiple objects, by keeping track of separate ballot numbers for each object. Vertical Paxos requires three separate WAN communications to change the leadership, while WPaxos can do so with just one WAN communication.

% Both protocols also suffer from increased number of communication steps when more than one node competes for leadership of the same object. 


\begin{figure}[t]
\centering
\includegraphics[width=50mm]{figures/vert_paxos.pdf}
\caption{Object stealing with Vertical Paxos requires a reconfiguration. (1) New Leader $L_n$ requests Master for next ballot $nb$. (2) $L_n$ receives $nb$ and $b$. (3) and (4) $L_n$ uses $b$ to locate configuration with such ballot and perfroms phase-1 of Paxos in the old configuration. (5) $L_n$ commits unfinished the slots learned in phase-1 and sends $complete$ message to Master. (6) master activates the configuration, so $L_n$ can start serving requests. }
\label{fig:vert_paxos}
\end{figure}


